On the effectiveness of virtualization-based security

Protecting commodity operating systems and applications against malware and targeted attacks has proven to be difficult. In recent years, virtualization has received attention from security researchers who utilize it to harden existing systems and provide strong security guarantees. This has lead to interesting use cases such as cloud computing where possibly sensitive data is processed on remote, third party systems. The migration and processing of data in remote servers, poses new technical and legal questions, such as which security measures should be taken to protect this data or how can it be proven that execution of code wasn't tampered with. In this paper we focus on technological aspects. We discuss the various possibilities of security within the virtualization layer and we use as a case study \HelloRootkitty{}, a lightweight invariance-enforcing framework which allows an operating system to recover from kernel-level attacks. In addition to \HelloRootkitty{}, we also explore the use of special hardware chips as a way of further protecting and guaranteeing the integrity of a virtualized system.

==> related.tex <==
A number of efforts exist on detecting and preventing kernel malware. 
In this section we explore related work that attempts to protect
a kernel using specialized hardware, virtualization, code integrity and
profiling.

\textbf{Hardware-based countermeasures} \label{hardware}
Copilot \cite{copilot} is a kernel integrity monitor which detects illegal
modiﬁcations to a host’s kernel by fetching physical memory pages where kernel
data and code is stored. Although the monitor has negligible overhead, it needs a separate PCI-card to fetch pages of the running kernel.
Gibraltar \cite{6} is a system to infer kernel data structure invariants by fetching snapshots of kernel memory in a way similar to Copilot, by using a PCI-card. The violation of the inferred invariants is reported as a potential attack. 
While detecting malicious behavior, those countermeasures are limited by the usage of special hardware. A wide deployment of such systems is harder to achieve. 

\textbf{Kernel code integrity} \label{integrity}
A countermeasure specifically designed to prevent the execution of unauthorized code is described in \cite{SecVisor}. The system comes in the form of a tiny hypervisor which protects legacy OSes and ensures that only validated code of the guest can execute in kernel mode. 
Another rootkit prevention system is NICKLE \cite{NICKLE}, which prevents
unauthorized kernel code execution via memory shadowing. The hypervisor
maintains a shadow physical memory to store authenticated guest kernel code. At
runtime it determines if the instruction fetch is for kernel or user mode. After
verifying the code it will route the instruction fetch accordingly to shadow or
standard memory. Kernel rootkit attacks would be detected and prevented since invalidated code would attempt to run in kernel mode.   

A recent attack to bypass countermeasures against code injection attacks,
such as the Non-Executable stack countermeasure, is Return Oriented Programming (ROP) \cite{geometry}. 
In ROP, the attacker, instead of injecting malicious code in the address space of a vulnerable process, crafts his malicious payload by combining fragments of existing code.
This method of attacking has been used to create return-oriented rootkits which
re-use fragments of authorized kernel code for malicious purposes
\cite{Hund2009}. Such rootkits can bypass countermeasures like the ones proposed by \cite{NICKLE,SecVisor}.\\
Yin et al. \cite{hookscout} protect kernel function pointers from being compromised by rootkits. The approach consists of an analysis and a detection subsystems. The analysis subsystem keeps track of function pointer propagation in kernel memory via a whole-system emulator and generates the policy for hook detection. The detection subsystem resides on the target machine and detects violations of the inferred policy. Although the described countermeasure is binary-centric and can generate a hook detection policy without modifying any guest source code, it can be disabled by a rootkit attack since the detection system resides in the target machine.
A countermeasure which protects kernel hooks dynamically allocated from the heap is described in \cite{HookSafe}. Since protection of kernel objects needs byte-level granularity, obviously finer than the page-level granularity provided by commodity hardware, this countermeasure relocates kernel hooks to be protected to a dedicated page and then exploits the regular page-level protection of the MMU. Although the overhead is negligible, rootkit attacks that compromise non-control data would not be prevented.

\textbf{Analysis and profiling systems} \label{profiling}
Malware analysis can reveal important information about the way a rootkit
compromises data structures or how private data are stolen, allowing researchers to understand rootkit's behavior and design effective countermeasures. 
A virtual machine monitor designed for malware analysis as described in
\cite{MAVMM} extracts features like memory pages, system calls, disk and network
accesses from the analyzed program running in the guest.
Wang et al. \cite{hookmap} is an analysis tool against persistent rootkits, which compromise kernel hooks for hiding purposes. Those kernel hooks are first identified by monitoring the kernel-side execution path of system utility programs (e.g. ps, ls) and then reported as potential targets.
Identification of kernel hooks and extraction of the hook implanting mechanisms
via dynamic analysis is proposed in \cite{hookfinder}. A whole-system emulator
is used rather than a virtual machine monitor. 
A rootkit proﬁler is described in \cite{PoKer}. A VMM is used to log the rootkit hooking behavior, to
monitor targeted kernel objects, to extract kernel rootkit code and infer the potential impact on user-level programs.

\emph{Hello rootKitty} can be easily integrated with the systems described above in
order to perform integrity checking and detect illegal changes to those kernel
objects collected by the analysis tools.

